Is Data All That Matters? The Role of Control Frequency for Learning-Based Sampled-Data Control of Uncertain Systems

Learning models or control policies from data has become a powerful tool to improve the performance of uncertain systems. While a strong focus has been placed on increasing the amount and quality of data to improve performance, data can never fully eliminate uncertainty, making feedback necessary to ensure stability and performance. We show that the control frequency at which the input is recalculated is a crucial design parameter, yet it has hardly been considered before. We address this gap by combining probabilistic model learning and sampled-data control. We use Gaussian processes (GPs) to learn a continuous-time model and compute a corresponding discrete-time controller. The result is an uncertain sampled-data control system, for which we derive robust stability conditions. We formulate semidefinite programs to compute the minimum control frequency required for stability and to optimize performance. As a result, our approach enables us to study the effect of both control frequency and data on stability and closed-loop performance. We show in numerical simulations of a quadrotor that performance can be improved by increasing either the amount of data or the control frequency, and that we can trade off one for the other. For example, by increasing the control frequency by 33%, we can reduce the number of data points by half while still achieving similar performance.

==> chapters/old_3_gp.tex <==
\section{Learning the Dynamics} %\label{sec:gp}
We employ Gaussian process (GP) regression to learn the unknown component of the dynamics in~\eqref{eq:prob_open_loop_system}. In this section, we summarize some fundamental properties of GPs and discuss their use to learn the dynamics model from data and to obtain a local linear approximation of the true system dynamics.

\subsection{Gaussian Process Regression} %\label{sec:gp_intro}
To simplify the notation, consider first the one-dimensional case, i.e., training samples ${y^{(i)}=g(\bm{z}^{(i)})+w^{(i)}}$, ${i=1,\dots,N}$ obtained through evaluation of an unknown function ${g:\R^{n_z}\rightarrow \R}$, with observation noise ${w^{(i)}\sim \mathcal{N}(0,\sigma_\mathrm{n}^2)}$, are available. 
GP regression~\cite{Rasmussen.2006} is based on the assumption that the unknown function is drawn from a GP. 
A GP induces a distribution $\mathcal{GP}(\mu(\cdot),k(\cdot,\cdot))$ over functions, such that any finite number of function evaluations is jointly Gaussian distributed.
The prior mean function $\mu:\R^{n_z}\rightarrow \R$ can incorporate prior knowledge in the form of an approximate model, and the kernel $k:\R^{n_z}\times\R^{n_z} \rightarrow \R$ encodes information about the structure of the unknown function. Without loss of generality, we set the mean function to zero, as prior knowledge is already incorporated through the definition of the training targets in~\eqref{prob:eq_dataset_assumption}.
Under the GP assumption, the function value at a test point $\bm{z}^*\in\R^{n_z}$ and the observed targets, stacked into a vector $\bm{y}=\big[y^{(1)},\dots,y^{(N)}\big]\tp$, have the joint probability distribution
\begin{align}
    \label{gp:joint_pd}
    \begin{bmatrix}
        \bm{y} \\ g(\bm{z}^*)
    \end{bmatrix} \sim
    \mathcal{N} \left(\bm{0}, \begin{bmatrix}
        \bmb{K} & \bm{k}(\bm{z}^*)\tp \\
        \bm{k}(\bm{z}^*) & k(\bm{z}^*,\bm{z}^*)
    \end{bmatrix} \right),
\end{align}
where the kernel vector and the data covariance matrix are defined as $\bm{k}(\bm{z}^*) = \big[k(\bm{z}^{(1)},\bm{z}^*),\dots,k(\bm{z}^{(N)},\bm{z}^*)\big]\tp$ and $\bmb{K}=\bm{K} + \sigma_\mathrm{n}^2 \bm{I}_n$, where $\bm{K}_{ij}=\big[k(\bm{z}^{(i)},\bm{z}^{(j)})\big]$.
By conditioning $g(\bm{z}^*)$ on the training data, we obtain the posterior distribution ${g(\bm{z}^*)\sim \mathcal{N}(\mu(\bm{z}^*),\sigma^2(\bm{z}^*))}$ with the predictive mean and variance
\begin{align}
    \label{eq:gp_posterior_mean}
    \mu(\bm{z}^*) &= \bm{k}(\bm{z}^*)\tp \bmb{K}^{-1} \bm{y} \\
    \label{eq:gp_posterior_variance}
    \sigma^2(\bm{z}^*) &= k(\bm{z}^*,\bm{z}^*) - \bm{k}(\bm{z}^*)\tp\bmb{K}^{-1} \bm{k}(\bm{z}^*).
\end{align}
The kernel function is usually parameterized by a set of hyperparameters which can be determined, e.g., by maximizing the marginal log-likelihood of the training data \cite{Rasmussen.2006}.

Since the derivative is a linear operator, the derivative of a GP is also a GP \cite{Rasmussen.2006}. From~\eqref{gp:joint_pd}, we obtain
\begin{align}
    \begin{bmatrix}
        \bm{y} \\ \left.\frac{\partial g(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*}
    \end{bmatrix} \sim
    \mathcal{N} \left(\bm{0}, \begin{bmatrix}
        \bmb{K} & \left.\frac{\partial \bm{k}(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*} \\
        \left.\frac{\partial \bm{k}(\bm{z})\tp}{\partial \bm{z}}\right|_{\bm{z}^*} & \left.\frac{\partial^2 k(\bm{z},\bm{z})}{\partial \bm{z} \partial \bm{z}} \right|_{\bm{z}^*}
    \end{bmatrix} \right).
\end{align}
Similar to the prediction of the function value at $\bm{z}^*$, predictions of the derivatives are obtained via conditioning as ${\left.\frac{\partial g(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*} \sim \mathcal{N}(\bm{\mu}'(\bm{z}^*),\bm{\Sigma}'(\bm{z}^*))}$ 
with
\begin{align}
    \label{eq:gp_mean_derivative}
    \bm{\mu}'(\bm{z}^*) &= 
    \left. \frac{\partial \bm{k}(\bm{z})}{\partial \bm{z}} \right|_{\bm{z}^*} \bm{\bar{K}}^{-1} \bm{y}, \\
    \label{eq:gp_variance_derivative}
    \bm{\Sigma}'(\bm{z}^*) &= 
    \left.\frac{\partial^2 k(\bm{z},\bm{z})}{\partial \bm{z} \partial \bm{z}} \right|_{\bm{z}^*} 
    \!\!- \left.\frac{\partial \bm{k}(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*} \!\!\bm{\bar{K}}^{-1} \left(\left.\frac{\partial \bm{k}(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*} \right)\tp.
\end{align}
These fundamental properties of GPs allow to learn an uncertain model of the model~\eqref{eq:prob_open_loop_system} and a locally valid linearization from the dataset~\eqref{prob:eq_dataset_assumption}, as discussed in the following.


\subsection{Model Learning and Linearization}
For compactness, we write the argument of the unknown function $\bm{g}$ as $\bm{z}=(\bm{x},\bm{u})$. 
For each output dimension of $\bm{g}$, independent GP regression models ${g_i(\cdot)\sim\mathcal{N}(\mu_i(\cdot), \sigma_i^2(\cdot))}$, ${i=1,\dots,n}$, are trained. 
This approach is common as it greatly reduces the computational complexity; however, it cannot capture possible correlations between the output dimensions of $\bm{g}$.
As the kernel, we use the popular squared-exponential (SE) function
\begin{align}
    \label{eq:gp_se_kernel}
    k(\bm{z},\bm{z}') &= \sigma_f^2 \exp{\left(-\frac{1}{2}(\bm{z}-\bm{z}')\tp \bm{L}^{-2}(\bm{z}-\bm{z}')\right)},
\end{align}
where $\sigma_f^2$ is the output variance and $\bm{L}=\mathrm{diag}(\bm{l})$ contains the length scales $\bm{l}=[l_1,\dots,l_{n+m}]$, which correspond to the rate of change of $\bm{g}$ w.r.t. $\bm{z}$.
The choice~\eqref{eq:gp_se_kernel} is not restrictive in practice since the corresponding space of sample functions of the GP contains all continuous functions \cite{Lederer.2019}.
For the SE kernel~\eqref{eq:gp_se_kernel}, the partial derivatives in~\eqref{eq:gp_mean_derivative} and~\eqref{eq:gp_variance_derivative} are straightforward to evaluate.
% given by
% \begin{align}
%     \label{eq:gp_se_kernel_first_derivative}
%     \left.\frac{\partial \bm{k}(\bm{z})}{\partial \bm{z}} \right|_{\bm{z}^*} &= \bm{L}^{-2}\begin{bmatrix}
%         (\bm{z}^{(1)}-\bm{z}^*)\tp k(\bm{z}^*,\bm{z}^{(1)}) \\ \vdots \\ (\bm{z}^{(N)}-\bm{z}^*)\tp k(\bm{z}^*,\bm{z}^{(N)})
%     \end{bmatrix}, \\
%     \label{eq:gp_se_kernel_second_derivative}
%     \left.\frac{\partial^2 k(\bm{z},\bm{z})}{\partial \bm{z} \partial \bm{z}} \right|_{\bm{z}^*} &=
%     \sigma_f^2 \bm{L}^{-2}.
% \end{align}

We linearize the dynamics around the operating point $\bm{z}^* = (\bm{x}_\mathrm{s},\bm{u}_\mathrm{s})$  via~\eqref{eq:gp_mean_derivative},~\eqref{eq:gp_variance_derivative}, and denote the derivative of the $i$-th GP by $\left.\frac{\partial g_i(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*}\sim \mathcal{N}(\bm{\mu}_i'(\bm{z}^*),\bm{\Sigma}_i'(\bm{z}^*))$.
The nominal learned linearized model is given by
\begin{align}
    \label{eq:gp_linearized_model_nominal}
    \begin{bmatrix}
        \bm{A} & \bm{B}
    \end{bmatrix} = \left.\frac{\partial \bm{f}(\bm{z})}{\partial \bm{z}} \right|_{\bm{z}^*} + 
    \begin{bmatrix}
        \bm{\mu}_1'(\bm{z}^*)\tp \\ \vdots \\ \bm{\mu}_n'(\bm{z}^*)\tp
    \end{bmatrix}.
\end{align}
%In \cite{Berkenkamp.2015}, confidence intervals for $\bm{A}$ and $\bm{B}$ are computed solely from the diagonal entries of $\bm{\Sigma}_i'(\bm{z}^*)$, which is inaccurate if the components of $\left.\frac{\partial g_i(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*}$ are correlated. 
Due to the properties of multivariate Gaussian distributions,
\begin{align}
    P\left(\left.\frac{\partial g_i(\bm{z})}{\partial \bm{z}}\right|_{\bm{z}^*} - \bm{\mu}_i'(\bm{z}^*) \in \mathcal{E}_i\right) = p,
\end{align}
with the ellipsoidal confidence region
\begin{align}
    \mathcal{E}_i = \left\{\bm{d} \in \R^{n+m}\left|\bm{d}\tp \left(\bm{\Sigma}_i'(\bm{z}^*)
    \right)^{-1}\bm{d} \leq \chi_{n+m}^2(p) \right. \right\},
\end{align}
where $\chi_{n+m}^2$ is the quantile function of the chi-squared distribution with $n+m$ degrees of freedom. It follows through computation of the bounding box of $\mathcal{E}_i$ that with probability of at least $p^n$, the true linearized dynamics are captured by
\begin{align}
    \label{eq:gp_uncertain_system1}
    \bm{\dot{x}} = (\bm{A} + \bmh{A} \circ \bm{\Omega}) \bm{x} +
    (\bm{B} + \bmh{B} \circ \bm{\Psi}) \bm{u},
\end{align}
where $\circ$ denotes the Hadamard (element-wise) product,
\begin{align}
    \label{eq:gp_linearized_model_uncertainty}
    \begin{bmatrix}
        \bmh{A} & \bmh{B}
    \end{bmatrix} = \gamma
    \begin{bmatrix}
        \sqrt{\mathrm{diag}(\bm{\Sigma}_1'(\bm{z}^*))} \\ \vdots \\ \sqrt{\mathrm{diag}(\bm{\Sigma}_n'(\bm{z}^*))}
    \end{bmatrix}
\end{align}
with $\gamma=\sqrt{\chi_{n+m}^2(p)}$, and ${\bm{\Omega} \in [-1,1]^{n \times n}}$, ${\bm{\Psi} \in [-1,1]^{n \times m}}$ are interval uncertainties. 
% and the corresponding uncertainty is 
% \begin{align}
%     \label{eq:gp_linearized_model_uncertainty}
%     \begin{bmatrix}
%         \bmh{A} & \bmh{B}
%     \end{bmatrix} = \gamma
%     \begin{bmatrix}
%         \sqrt{\mathrm{diag}(\bm{\Sigma}_1'(\bm{z}^*))} \\ \vdots \\ \sqrt{\mathrm{diag}(\bm{\Sigma}_n'(\bm{z}^*))}
%     \end{bmatrix},
% \end{align}
% where $\mathrm{diag}(\bm{\Sigma})$ is a row vector consisting of the diagonal elements of $\bm{\Sigma}$, and $\sqrt{\cdot}$ acts element-wise. The matrices $\bmh{A}=\big[\bmh{a}_1\,\dots\,\bmh{a}_n\big]\tp$ and $\bmh{B}=\big[\bmh{b}_1\,\dots\,\bmh{b}_n\big]\tp$ represent confidence intervals for the elements in $\bm{A}$ and $\bm{B}$. For a sufficiently large value of $\gamma$, e.g., $\gamma=3$ (99.7\% confidence), the true linearized dynamics are captured with high probability by

%\subsection{Uncertainty Reparameterization}
To be able to incorporate the model uncertainty in a robust sampled-data controller design, we have to reparameterize the terms in~\eqref{eq:gp_uncertain_system1} corresponding to the model uncertainty. For this, we make use of the following proposition, which is straightforward to prove.
\begin{proposition} \label{prop:unc_reparameterization_trick}
    Let ${\bm{X}\! =\! \big[\bm{x}_1\, \dots\, \bm{x}_n\big]\tp\! \in\! \R^{n \times n}, {\bm{Y}\! \in \!\R^{n \times n}}}$. Then, the Hadamard product $\bm{X} \circ \bm{Y}$ can expressed as 
    \begin{align}
        \bm{X}\! \circ\! \bm{Y} = (\bm{I}_n \otimes \bm{1}_{1\times n}) \mathrm{Diag}\left(\mathrm{vec}\left(\bm{Y}\tp\right)\right) \!\begin{bmatrix}
            \mathrm{Diag}(\bm{x}_1) \\ \vdots \\ \mathrm{Diag}(\bm{x}_n)
        \end{bmatrix}\!,\! 
    \end{align}
    where $\otimes$ denotes the Kronecker product and $\mathrm{vec}(\bm{Y}\tp) \in \R^{n^2}$ is the vectorization of $\bm{Y}\tp$.
\end{proposition}

As a result of Proposition~\ref{prop:unc_reparameterization_trick}, the uncertain terms in~\eqref{eq:gp_uncertain_system1} can be written as
\begin{align}
    \label{eq:gp_uncertainty_reparameterization}
    \bmh{A} \circ \bm{\Omega} = \bm{H}\bm{\Delta}\bm{E}, \qquad \bmh{B} \circ \bm{\Psi} = \bm{H}\bm{\Delta}\bm{F},
\end{align}
where ${\bm{\Delta}=\mathrm{Diag}([\delta_1,\dots,\delta_p])}$ with $|\delta_i|\leq 1$, $i=1,\dots,p$, $p=n^2+nm$, $\bm{H} = \big[\bm{I}_n \otimes \bm{1}_{1 \times n}, \bm{I}_n \otimes \bm{1}_{1 \times m}]$, and
\begin{align}
    \bm{E} = \begin{bmatrix}
        \mathrm{Diag}(\bmh{a}_1) \\ \vdots \\ \mathrm{Diag}(\bmh{a}_n) \\ \bm{0}_{nm \times n}
    \end{bmatrix}, \quad 
    \bm{F} = \begin{bmatrix}
        \bm{0}_{n^2 \times n} \\
        \mathrm{Diag}(\bmh{b}_1) \\ \vdots \\ \mathrm{Diag}(\bmh{b}_n)
    \end{bmatrix}.
\end{align}
In the following section, we discuss how this uncertainty representation can be used to design a sampled-data controller.

==> chapters/old_4_sampled_data.tex <==
\section{Robust Sampled-Data Control} \label{sec:sd}
By inserting the uncertainty representation~\eqref{eq:gp_uncertainty_reparameterization} into~\eqref{eq:gp_uncertain_system1}, we obtain the uncertain linearized system
\begin{align}
    \label{eq:sd_norm_bounded_open_loop_system}
    \bm{\dot{x}}(t) = (\bm{A} + \bm{H}\bm{\Delta}\bm{E})\bm{x}(t) + (\bm{B} + \bm{H}\bm{\Delta}\bm{F})\bm{u}(t),
\end{align}
where $\bm{\Delta} \in \R^{p \times p}$ is an unknown matrix satisfying ${\bm{\Delta}\tp \bm{\Delta} \preceq \bm{I}}$, and $\bm{H} \in \R^{n \times p}, \bm{E} \in \R^{p \times n}, \bm{F} \in \R^{p \times m}$ are known. As the sampled-data control law~\eqref{eq:prob_input}, we employ the linear state feedback
\begin{align}
    \label{eq:sd_control_law_lin}
    \bm{u}(t) = \bm{K}\bm{x}(t_k), \qquad t_k \leq t < t_{k+1},
\end{align}
where $\bm{K}\in \R^{m \times n}$ is the gain matrix.
Hence, the closed-loop linearized sampled-data control system can be written as
\begin{align}
    \label{eq:sd_norm_bounded_closed_loop_system}
    \!\!\bm{\dot{x}}(t)\! =\! (\bm{A}\! +\! \bm{H}\bm{\Delta}\bm{E})\bm{x}(t)\! + \!(\bm{B}\! +\! \bm{H}\bm{\Delta}\bm{F})\bm{K}\bm{x}(t\! -\! \tau(t)),\!\!
\end{align}
where ${\tau(t) = t-t_k}$ is a piecewise-continuous, time-varying delay. As a result of Assumption~\ref{ass:sd_sampling_interval}, the delay is bounded by ${\tau(t)\in[0,T_\mathrm{s}]}$, $\forall t$. 

\subsection{Robust Stabilization}
Numerous results exist for the stability of linear systems with an upper bound on the delay. We focus on the stability conditions stated in \cite{Fridman.2004}, which are based on the Lyapunov-Krasovskii functional
\begin{align}
    \label{eq:sd_lyapunov_functional}
    V = \bm{x}(t)\tp \bm{Q}_1 \bm{x}(t) + \int_{-T_\mathrm{s}}^0 \int_{t+\theta}^t \bmd{x}(s)\tp \bm{R} \bmd{x}(s) \mathrm{d}s \mathrm{d} \theta,
\end{align}
where $\bmb{Q}_1 \succ \bm{0}$ and $\bm{R}\succ \bm{0}$. Defining $\bm{Q}_1 = \bmb{Q}_1^{-1}$, $\bmb{R} = \bm{R}_1^{-1}$, the following stability conditions are derived in \cite{Fridman.2004} for the nominal sampled-data system
\begin{align}
    \label{eq:sd_nominal_open_loop_system}
    \bm{\dot{x}}(t) = \bm{A}\bm{x}(t) + \bm{B}\bm{u}(t).
\end{align}
\begin{lemma} \label{lem:sd_nominal_step2}
    {\normalfont \cite{Fridman.2004}}
    The control law~\eqref{eq:sd_control_law_lin} stabilizes system~\eqref{eq:sd_nominal_open_loop_system} for all samplings satisfying Assumption~\ref{ass:sd_sampling_interval} if there exist matrices $\bm{Q}_1 \succ \bm{0}, \bm{Q}_2, \bm{Q}_3, \bmb{Z}_1, \bmb{Z}_2, \bmb{Z}_3, \bmb{R} \succ \bm{0}$, all in $\R^{n \times n}$, and ${\bmb{Y} \in \R^{m \times n}}$, that satisfy the LMIs
    \begin{align}
        \label{eq:sd_nominal_lmi3}
        \begin{bmatrix}
            \bm{\Xi}_1 & \bm{\Xi}_2 & T_\mathrm{s}\bm{Q}_2\tp \\
            * & -\bm{Q}_3 - \bm{Q}_3\tp + T_\mathrm{s}\bmb{Z}_3 & T_\mathrm{s}\bm{Q}_3\tp \\
            * & * & -T_\mathrm{s}\bmb{R} 
        \end{bmatrix} \prec \bm{0}, \\
        \label{eq:sd_nominal_lmi4}
        \begin{bmatrix}
            \bm{Q}_1 \bmb{R}^{-1}\bm{Q}_1 & \bm{0} & \bmb{Y}\tp \bm{B}\tp \\
            * & \bmb{Z}_1 & \bmb{Z}_2 \\
            * & * & \bmb{Z}_3
        \end{bmatrix} \succeq \bm{0},
    \end{align}
    where ${\bm{\Xi}_1 = \bm{Q}_2 + \bm{Q}_2\tp + T_\mathrm{s} \bmb{Z}_1}$ and $\bm{\Xi}_2=\bm{Q}_3 - \bm{Q}_2\tp + \bm{Q}_1\bm{A}\tp + T_\mathrm{s}\bmb{Z}_2 + \bmb{Y}\tp \bm{B}\tp$. The state-feedback gain is then given by $\bm{K}=\bmb{Y}\bm{Q}_1^{-1}$. 
\end{lemma}

The above result can also be directly applied to the case of polytopic uncertainty, but not to the norm-bounded uncertainty~\eqref{eq:gp_uncertainty_reparameterization} of the linearized GP dynamics model. To overcome this problem, we make use of the following proposition \cite{Xie.1996}.
\begin{proposition} \label{prop:sd_norm_bounded_trick}
    {\normalfont{\cite{Xie.1996}}}
    Let $\bm{\Delta}\tp \bm{\Delta} \preceq \bm{I}$. Then, for all scalars $\epsilon > 0$ and all constant matrices $\bm{M}$, $\bm{N}$ of appropriate dimension, it holds that
    \begin{align}
    \begin{split}
        -\epsilon^{-1}\bm{M}\bm{M}\tp - \epsilon \bm{N}\tp \bm{N} 
        &\preceq \bm{M}\bm{\Delta} \bm{N} + \bm{N}\tp \bm{\Delta}\tp\bm{M}\tp \\
        &\preceq \epsilon^{-1}\bm{M}\bm{M}\tp + \epsilon \bm{N}\tp \bm{N}.
    \end{split}
    \end{align}
\end{proposition}

\begin{theorem} \label{the:sd_norm_bounded_step2}
    The control law~\eqref{eq:sd_control_law_lin} stabilizes the uncertain system~\eqref{eq:sd_norm_bounded_open_loop_system} for all samplings satisfying Assumption~\ref{ass:sd_sampling_interval} if there exist matrices $\bm{Q}_1 \succ \bm{0}, \bm{Q}_2, \bm{Q}_3, \bmb{Z}_1, \bmb{Z}_2, \bmb{Z}_3, \bmb{R} \succ \bm{0}$, all in $\R^{n \times n}$, ${\bmb{Y} \in \R^{m \times n}}$, and scalars $\epsilon_1 > 0$, $\epsilon_2 > 0$, that satisfy the matrix inequalities
    \begin{align}
        \label{eq:sd_norm_bounded_lmi3}
        \begin{bmatrix}
            \multicolumn{3}{c}{\multirow{3}{*}{\bm{W}}} & \bm{0} & \epsilon_1(\bm{Q}_1\bm{E}\tp + \bmb{Y}\tp\bm{F}\tp) \\
            \multicolumn{3}{c}{} & \bm{H} & \bm{0} \\
            \multicolumn{3}{c}{} & \bm{0} & \bm{0} \\
            * & * & * & -\epsilon_1 \bm{I} & \bm{0} \\
            * & * & * & * & -\epsilon_1 \bm{I}
        \end{bmatrix} &\prec \bm{0}, \\
        \label{eq:sd_norm_bounded_lmi4}
        \begin{bmatrix}
            2\bm{Q}_1 - \bmb{R} & \bm{0} & \bmb{Y}\tp \bm{B}\tp & \bm{0} & \epsilon_2 \bmb{Y}\tp \bm{F}\tp \\
            * & \bmb{Z}_1 & \bmb{Z}_2 & \bm{0} & \bm{0} \\
            * & * & \bmb{Z}_3 & \bm{H} & \bm{0} \\
            * & * & * &  \epsilon_2 \bm{I} & \bm{0} \\
            * & * & * & * & \epsilon_2 \bm{I}
        \end{bmatrix} &\succeq \bm{0},
    \end{align}
    where $\bm{W}$ denotes the LHS of~\eqref{eq:sd_nominal_lmi3}. The state-feedback gain is then given by $\bm{K}=\bmb{Y}\bm{Q}_1^{-1}$. 
\end{theorem}


\begin{proof}
    We replace $\bm{A}$ and $\bm{B}$ in~\eqref{eq:sd_nominal_lmi3} by $\bm{A}+\bm{H}\bm{\Delta}\bm{E}$ and $\bm{B}+\bm{H}\bm{\Delta}\bm{F}$, respectively, and obtain
    \begin{align}
        &\begin{bmatrix}
                \bm{\Xi}_1 & \bm{\Xi}_2 + \bm{Q}_1(\bm{H}\bm{\Delta}\bm{E})\tp + \bmb{Y}\tp(\bm{H}\bm{\Delta}\bm{F})\tp & T_\mathrm{s}\bm{Q}_2\tp \\
                * & -\bm{Q}_3 - \bm{Q}_3\tp + T_\mathrm{s}\bmb{Z}_3 & T_\mathrm{s}\bm{Q}_3\tp \\
                * & * & -T_\mathrm{s}\bmb{R} 
        \end{bmatrix} \nonumber \\
        =&\; \bm{W} + \begin{bmatrix}
            \bm{0} & \bm{Q}_1 \bm{E}\tp \bm{\Delta}\tp \bm{H}\tp + \bmb{Y}\tp \bm{F}\tp \bm{\Delta}\tp \bm{H}\tp & \bm{0} \\
            * & \bm{0} & \bm{0} \\
            * & * & \bm{0}
        \end{bmatrix} \nonumber \\
        =&\; \bm{W} + \bm{M} \bm{\Delta} \bm{N} + \bm{N}\tp \bm{\Delta}\tp \bm{M}\tp \prec \bm{0},
        \label{eq:proof1}
    \end{align}
    where $\bm{M}=\begin{bmatrix} \bm{0} & \bm{H}\tp & \bm{0} \end{bmatrix}\tp$ and $\bm{N}=\begin{bmatrix} \bm{E}\bm{Q}_1\tp + \bm{F} \bmb{Y} & \bm{0} & \bm{0} \end{bmatrix}$.
    Applying Proposition~\ref{prop:sd_norm_bounded_trick} to the second and third term in~\eqref{eq:proof1} yields
    \begin{align}
        & \bm{W} + \bm{M} \bm{\Delta} \bm{N} + \bm{N}\tp \bm{\Delta}\tp \bm{M}\tp \\
        \preceq \; & \bm{W} + \epsilon_1^{-1} \bm{M} \bm{M}\tp + \epsilon_1 \bm{N}\tp \bm{N} \\
        =\;& \bm{W} + 
        \begin{bmatrix} 
            \bm{M} & \epsilon_1\bm{N}\tp 
        \end{bmatrix}
        \begin{bmatrix}
            \epsilon_1^{-1} \bm{I} & \bm{0} \\ 
            \bm{0} & \epsilon_1^{-1} \bm{I}
        \end{bmatrix}
        \begin{bmatrix}
            \bm{M}\tp \\
            \epsilon_1\bm{N}
        \end{bmatrix} \prec \bm{0},
    \end{align}
    for all scalars $\epsilon_1 > 0$. Application of the Schur complement~\cite{Boyd.1994} and inserting the definitions of $\bm{M}$ and $\bm{N}$ gives~\eqref{eq:sd_norm_bounded_lmi3}. To obtain the second LMI~\eqref{eq:sd_norm_bounded_lmi4}, we replace $\bm{B}$ in~\eqref{eq:sd_nominal_lmi4} by $\bm{B}+\bm{H}\bm{\Delta}\bm{F}$ and proceed in a similar way as above, which yields the nonlinear matrix inequality
    \begin{align}
        \label{eq:sd_norm_bounded_lmi4_bilinear}
        \begin{bmatrix}
            \bm{Q}_1 \bmb{R}^{-1}\bm{Q}_1 & \bm{0} & \bmb{Y}\tp \bm{B}\tp & \bm{0} & \epsilon_2 \bm{Y}\tp \bm{F}\tp \\
            * & \bmb{Z}_1 & \bmb{Z}_2 & \bm{0} & \bm{0} \\
            * & * & \bmb{Z}_3 & \bm{H} & \bm{0} \\
            * & * & * &  \epsilon_2 \bm{I} & \bm{0} \\
            * & * & * & * & \epsilon_2 \bm{I}
        \end{bmatrix} &\succeq \bm{0}.
    \end{align}
    To replace the nonlinear term $\bm{Q}_1 \bmb{R}^{-1}\bm{Q}_1$, we make use of the fact that $\bmb{R}=\bmb{R}\tp$ implies
    \begin{gather}
        (\bm{Q}_1 - \bmb{R})\tp\bmb{R}^{-1}(\bm{Q}_1 - \bmb{R}) = \bm{Q}_1\tp\bmb{R}^{-1}\bm{Q}_1 - 2\bm{Q}_1 + \bmb{R} \succ \bm{0} \nonumber \\
        \Rightarrow \bm{Q}_1\tp\bmb{R}^{-1}\bm{Q}_1 \succ 2\bm{Q}_1 - \bmb{R}.
    \end{gather}
    It directly follows from application of the Schur complement that the holding of the LMI~\eqref{eq:sd_norm_bounded_lmi4} implies the holding of~\eqref{eq:sd_norm_bounded_lmi4_bilinear}, which concludes the proof.
\end{proof}

% \begin{figure*}[ht!]
%     \centering
%     \begin{align}
%     \label{eq:sd_gevp_lmi}
%     \begin{bmatrix}
%             \bmb{Z}_1 & \bmb{Z}_2 & \bm{Q}_2\tp & \bm{0} & \bm{0} \\
%             * & \bmb{Z}_3 & \bm{Q}_3\tp & \bm{0} & \bm{0} \\
%             * & * & -\bmb{R} & \bm{0} & \bm{0} \\
%             * & * & * & \bm{0} & \bm{0} \\
%             * & * & * & * & \bm{0}
%         \end{bmatrix} \prec -\frac{1}{T_\mathrm{s}} 
%         \begin{bmatrix}
%             \bm{Q}_2 + \bm{Q}_2\tp & \bm{Q}_3 - \bm{Q}_2\tp + \bm{Q}_1 \bm{A}\tp + \bmb{Y}\tp \bm{B}\tp & \bm{0} & \bm{0} & \epsilon_1(\bm{Q}_1 \bm{E}\tp + \bmb{Y}\tp \bm{F}\tp) \\
%             * & -\bm{Q}_3-\bm{Q}_3\tp & \bm{0} & \bm{H} & \bm{0} \\
%             * & * & \bm{0} & \bm{0} & \bm{0} \\
%             * & * & * & -\epsilon_1 \bm{I} & \bm{0} \\
%             * & * & * & * & -\epsilon_1 \bm{I}
%         \end{bmatrix}
%     \end{align} \\
%     \hline
%     \label{fig:gevp_lmi}
% \end{figure*}
Theorem~\ref{the:sd_norm_bounded_step2} allows to evaluate whether system~\eqref{eq:sd_norm_bounded_closed_loop_system} can be robustly stabilized by~\eqref{eq:sd_control_law_lin} for a given sampling time $T_\mathrm{s}$. Moreover, we can compute the MSI for system~\eqref{eq:sd_norm_bounded_closed_loop_system} by solving the optimization problem
\begin{align}
\begin{split}
\label{eq:sd_norm_bounded_stability_op}
    \min_{\substack{
            T_\mathrm{s}, \bm{Q}_1, \bm{Q}_2, \bm{Q}_3, \bmb{Z}_1, \\
            \bmb{Z}_2, \bmb{Z}_3, \bmb{R}, \bmb{Y}, \epsilon_1, \epsilon_2
        }}
    \quad & \frac{1}{T_\mathrm{s}} \\
    \text{s.t.} \qquad \quad & \bm{Q}_1 = \bm{Q}_1\tp \succ \bm{0}, \quad \bmb{R} = \bmb{R}\tp \succ \bm{0} \\
        &\eqref{eq:sd_norm_bounded_lmi3},
        \quad~\eqref{eq:sd_norm_bounded_lmi4}.
\end{split}
\end{align}
Problem~\eqref{eq:sd_norm_bounded_stability_op} represents a generalized eigenvalue minimization problem (GEVP) \cite{Boyd.1994}, which is a special type of SDPs that can be solved efficiently, e.g., with the bisection method \cite{Boyd.2004}. We denote the obtained MSI by $T_{\mathrm{s,max}} = \frac{1}{f_{\mathrm{c,min}}}$, where $f_{\mathrm{c,min}}$ is the minimum control frequency. 

\subsection{Performance Optimization}
For a chosen sampling time $T_\mathrm{s} \in (0,T_\mathrm{s,max}]$, we aim to optimize the system performance. For this, we consider the minimization of the cost function 
\begin{align}
    \label{eq:sd_cost}
    J = \int_{\tau_0}^{\tau_1} \bm{x}(t_k)\tp \bm{J}_1 \bm{x}(t_k) + \bm{u}(t)\tp \bm{J}_2 \bm{u}(t) \mathrm{d} t_k,
\end{align}
where $\tau_1 - \tau_0 \geq 0$ is the optimization period and $\bm{J}_1 \succ \bm{0}$, $\bm{J}_2 \succ \bm{0}$ are weight matrices. 
To make the problem tractable, we let ${J < \bar{J} = \eta \int_{\tau_0}^{\tau_1} \bm{x}(t_k)\tp \bm{Q}_1^{-1} \bm{Q}_1^{-1} \bm{x}(t_k)\mathrm{d} t_k}$ \cite{Lam.2006}, and consider the minimization of $\eta$. By inserting~\eqref{eq:sd_control_law_lin}, ${\bm{K}=\bmb{Y}\bm{Q}_1^{-1}}$, and applying the Schur complement, we obtain that $J<\bar{J}$ is equivalent to
\begin{align}
    \label{sd:cost_lmi}
    \begin{bmatrix}
        -\eta \bm{I} & \bm{Q}_1 & \bmb{Y}\tp \\ 
        * & -\bm{J}_1^{-1} & \bm{0} \\
        * & * & -\bm{J}_2^{-1}
    \end{bmatrix} \prec \bm{0}.
\end{align}
As a result, optimization of the performance while ensuring robust stability can be achieved by solving the GEVP
\begin{align}
\begin{split}
\label{eq:sd_norm_bounded_performance_op}
    \min_{\substack{
            \bm{Q}_1, \bm{Q}_2, \bm{Q}_3, \bmb{Z}_1, \\
            \bmb{Z}_2, \bmb{Z}_3, \bmb{R}, \bmb{Y}, \epsilon_1, \epsilon_2
        }}
    \quad & \eta \\
    \text{s.t.} \qquad \quad & \bm{Q}_1 = \bm{Q}_1\tp \succ \bm{0}, \quad \bmb{R} = \bmb{R}\tp \succ \bm{0} \\
        &~\eqref{eq:sd_norm_bounded_lmi3},\quad~\eqref{eq:sd_norm_bounded_lmi4}, \quad~\eqref{sd:cost_lmi},
\end{split}
\end{align}
for a given sampling time $T_\mathrm{s} \in \left(0,T_{\mathrm{s,max}}\right]$. The controller gain is again given by $\bm{K} = \bmb{Y}\bm{Q}_1^{-1}$.


==> chapters/things_to_add.tex <==
\begin{enumerate}
    \item Optimization over $\epsilon_1$ and $\epsilon_2$ can be simplified by setting $\epsilon_2 = \frac{1}{\epsilon_1}$.
\end{enumerate}
